Multilevel nested simulation for efficient risk estimation

We investigate the problem of computing a nested expectation of the form $\mathbb{P}[\mathbb{E}[X|Y] \!\geq\!0]\!=\!\mathbb{E}[\textrm{H}(\mathbb{E}[X|Y])]$ where $\textrm{H}$ is the Heaviside function. This nested expectation appears, for example, when estimating the probability of a large loss from a financial portfolio. We present a method that combines the idea of using Multilevel Monte Carlo (MLMC) for nested expectations with the idea of adaptively selecting the number of samples in the approximation of the inner expectation, as proposed by (Broadie et al., 2011). We propose and analyse an algorithm that adaptively selects the number of inner samples on each MLMC level and prove that the resulting MLMC method with adaptive sampling has an $\mathcal{O}\left( \varepsilon^{-2}|\log\varepsilon|^2 \right)$ complexity to achieve a root mean-squared error $\varepsilon$. The theoretical analysis is verified by numerical experiments on a simple model problem. We also present a stochastic root-finding algorithm that, combined with our adaptive methods, can be used to compute other risk measures such as Value-at-Risk (VaR) and Conditional Value-at-Risk (CVaR), with the latter being achieved with $\mathcal{O}\left(\varepsilon^{-2}\right)$ complexity.

==> imgs/model-max/err.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}

\begin{axis}[
xlabel={$\ell$},
ylabel={$E_\ell$},
xmin=0, xmax=14,
ymin=1e-08, ymax=0.01,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={0,2,4,6,8,10,12,14},
xticklabels={$0$,$2$,$4$,$6$,$8$,$10$,$12$,$14$},
ytick={1e-09,1e-08,1e-07,1e-06,1e-05,0.0001,0.001,0.01,0.1,1},
yticklabels={,$10^{-8}$,$10^{-7}$,$10^{-6}$,$10^{-5}$,$10^{-4}$,$10^{-3}$,$10^{-2}$,,},
tick pos=both
]

\addplot [mark=diamond, fixed error bar={x02}{y20}{y-err}]
table {\loadedtable};
\label{max_model_gpu/err-line0}

\addplot [dashed, mark=diamond, forget plot, fixed error bar={x02}{y21}{y-err01}]
table {\loadedtable};

\addplot [mark=square, fixed error bar={x02}{y22}{y-err02}]
table {\loadedtable};
\label{max_model_gpu/err-line1}

\addplot [dashed, mark=square, forget plot, fixed error bar={x02}{y23}{y-err03}]
table {\loadedtable};

\addplot [mark=*, fixed error bar={x02}{y24}{y-err04}]
table {\loadedtable};
\label{max_model_gpu/err-line2}

\addplot [dashed, mark=*, forget plot, fixed error bar={x02}{y25}{y-err05}]
table {\loadedtable};

\addplot [mark=triangle, fixed error bar={x02}{y26}{y-err06}]
table {\loadedtable};
\label{max_model_gpu/err-line3}

\addplot [dashed, mark=triangle, forget plot, fixed error bar={x02}{y27}{y-err07}]
table {\loadedtable};

\addplot [mark=asterisk, fixed error bar={x02}{y28}{y-err08}]
table {\loadedtable};
\label{max_model_gpu/err-line4}

\addplot [dashed, mark=asterisk, forget plot, fixed error bar={x02}{y29}{y-err09}]
table {\loadedtable};

\addplot [dashed, domain=0:16]
{%
0.0135353295278936 * 2^(-2*x)
};
\label{max_model_gpu/err-line6}

\coordinate (legend) at (axis description cs:0.03,0.03);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={south west}] at (legend) {
\ref{max_model_gpu/err-line6}& {$2^{ -2\ell }$}\\
};
\end{tikzpicture}


==> imgs/model-max/total_work.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}

\begin{axis}[
xlabel={Normalised \tol},
ylabel={Total work $\times \tol^2$},
xmin=5e-4, xmax=2e-1,
ymin=1, ymax=100,
xmode=log,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={0.001,0.01,0.1},
xticklabels={$10^{-3}$,$10^{-2}$,$10^{-1}$},
ytick={0.1,1,10,100,1000},
yticklabels={,$10^{0}$,$10^{1}$,$10^{2}$,},
tick pos=both
]
\addplot [mark=diamond]
table [x=x01, y=y10] {\loadedtable};
\label{max_model_gpu/total_work-line0}

\addplot [mark=square]
table [x=x01, y=y11] {\loadedtable};
\label{max_model_gpu/total_work-line1}

\addplot [mark=*]
table [x=x01, y=y12] {\loadedtable};
\label{max_model_gpu/total_work-line2}

\addplot [mark=triangle]
table [x=x01, y=y13] {\loadedtable};
\label{max_model_gpu/total_work-line3}

\addplot [mark=asterisk]
table [x=x01, y=y14] {\loadedtable};
\label{max_model_gpu/total_work-line4}
\addplot [dashed, domain=1e-04:10]
{ 8 };
\label{max_model_gpu/total_work-line9}
\coordinate (legend) at (axis description cs:0.03,0.97);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={north west}] at (legend) {
\ref{max_model_gpu/total_work-line9}& {$\tol^{ -2 }$}\\
};
\end{tikzpicture}


==> imgs/model-max/var.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}
\begin{axis}[
xlabel={$\ell$},
ylabel={$V_\ell$},
xmin=0, xmax=14,
ymin=1e-13, ymax=0.01,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={0,2,4,6,8,10,12,14},
xticklabels={$0$,$2$,$4$,$6$,$8$,$10$,$12$,$14$},
ytick={1e-14,1e-13,1e-12,1e-11,1e-10,1e-09,1e-08,1e-07,1e-06,1e-05,0.0001,0.001,0.01,0.1,1},
yticklabels={,$10^{-13}$,$10^{-12}$,$10^{-11}$,$10^{-10}$,$10^{-9}$,$10^{-8}$,$10^{-7}$,$10^{-6}$,$10^{-5}$,$10^{-4}$,$10^{-3}$,$10^{-2}$,,},
tick pos=both
]

\addplot [mark=diamond, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y30, y error=y-err10] {\loadedtable};
\label{max_model_gpu/var-line0}

\addplot [dashed, mark=diamond, forget plot, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y31, y error=y-err11] {\loadedtable};

\addplot [mark=square, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y32, y error=y-err12] {\loadedtable};
\label{max_model_gpu/var-line1}

\addplot [dashed, mark=square, forget plot, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y33, y error=y-err13] {\loadedtable};

\addplot [mark=*, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y34, y error=y-err14] {\loadedtable};
\label{max_model_gpu/var-line2}

\addplot [dashed, mark=*, forget plot, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y35, y error=y-err15] {\loadedtable};

\addplot [mark=triangle, fixed error bar={x02}{y36}{y-err16}]
table {\loadedtable};
\label{max_model_gpu/var-line3}

\addplot [dashed, mark=triangle, forget plot, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y37, y error=y-err17] {\loadedtable};

\addplot [mark=asterisk, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y38, y error=y-err18] {\loadedtable};
\label{max_model_gpu/var-line4}

\addplot [dashed, mark=asterisk, forget plot, error bars/.cd, y dir=both, y explicit]
table [x=x02, y=y39, y error=y-err19] {\loadedtable};

\addplot [dashed, domain=0:16]
{%
6e-04 * 2^(-3*x)
};
\label{max_model_gpu/var-line6}

\coordinate (legend) at (axis description cs:0.03,0.03);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={south west}] at (legend) {
\ref{max_model_gpu/var-line6}& {$2^{ -3\ell }$}\\
};
\end{tikzpicture}


==> imgs/model-max/work.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}

\begin{axis}[
xlabel={$\ell$},
ylabel={$\E{N_\ell}$},
xmin=0, xmax=14,
ymin=10, ymax=10000000,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={0,2,4,6,8,10,12,14},
xticklabels={$0$,$2$,$4$,$6$,$8$,$10$,$12$,$14$},
ytick={1,10,100,1000,10000,100000,1000000,10000000,100000000},
yticklabels={,$10^{1}$,$10^{2}$,$10^{3}$,$10^{4}$,$10^{5}$,$10^{6}$,$10^{7}$,},
tick pos=both
]
\addplot [mark=diamond]
table [x=x02, y=y40] {\loadedtable};
\label{max_model_gpu/work-line0}

\addplot [mark=square]
table [x=x02, y=y41] {\loadedtable};
\label{max_model_gpu/work-line1}

\addplot [mark=*]
table [x=x02, y=y42] {\loadedtable};
\label{max_model_gpu/work-line2}

\addplot [mark=triangle]
table [x=x02, y=y43] {\loadedtable};
\label{max_model_gpu/work-line3}

\addplot [mark=asterisk]
table [x=x02, y=y44] {\loadedtable};
\label{max_model_gpu/work-line4}

\addplot [dashed, domain=0:16]
{%
225.441634745356 * 2^x
};
\label{max_model_gpu/work-line6}
\coordinate (legend) at (axis description cs:0.97,0.03);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={south east}] at (legend) {
\ref{max_model_gpu/work-line6}& {$2^{ \ell }$}\\
};
\end{tikzpicture}


==> imgs/model-problem/functions.tex <==
\def\vartau{0.02}
\def\varLc{0.080477723746297747}

\tikzset{
  declare function={
    normcdf(\x)=1/(1 + exp(-0.07056*((\x))^3 - 1.5976*(\x)));
    normpdf(\x)= exp(-\x^2/2)/ sqrt(2*pi);
    distance(\x) = \vartau * (\x^2 - 1) - \varLc;
    sigma(\x) = sqrt(2. * \vartau ^ 2 + 4 * \vartau * (1 - \vartau) * (\x^2));
    signeddelta(\x) = distance(\x) / sigma(\x);
    signeddeltaderiv(\x) = 2*\vartau*\x / sigma(\x) -
     4 * signeddelta(\x) * \x *\vartau * (1-\vartau) / (sigma(\x))^2;
  },
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../../main"
%%% End:


==> imgs/root-finding/total-time.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}

\begin{axis}[
xlabel={Normalised $\tol$},
ylabel={Running time [s] $\times \tol^{2}$},
xmin=1e-05, xmax=0.1,
ymin=1e-08, ymax=1e-06,
xmode=log,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10},
xticklabels={,$10^{-5}$,$10^{-4}$,$10^{-3}$,$10^{-2}$,$10^{-1}$,,},
ytick={1e-09,1e-08,1e-07,1e-06,1e-05,0.0001},
yticklabels={,$10^{-8}$,$10^{-7}$,$10^{-6}$,,},
tick pos=both
]
\addplot [mark=*]
table {%
0.0970765528188712 1.3973403838454e-07
0.0485382764094356 4.38471640033157e-08
0.0242691382047178 2.40505414694645e-08
0.0121345691023589 1.6064643659755e-08
0.0121345691023589 3.10659250620568e-08
0.00606728455117945 1.75416535815647e-08
0.00606728455117945 3.12974700970581e-08
0.00303364227558973 2.1075934834419e-08
0.00151682113779486 2.48785210506465e-08
0.000758410568897431 2.56250060578025e-08
0.000379205284448716 3.12284566058116e-08
0.000189602642224358 3.27638711013433e-08
0.000189602642224358 5.76756134148755e-08
9.48013211120547e-05 4.26304021610243e-08
};
\label{root-finding/complexity-time-line0}
\addplot [dashed,domain=1e-6:1]
{%
%1e-05 7.23101581545742e-08
5.4554166562849734e-10*(ln(x))^2
};
\label{root-finding/complexity-time-line1}
\coordinate (legend) at (axis description cs:0.97,0.97);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={north east}] at (legend) {
\ref{root-finding/complexity-time-line1}& {$\varepsilon^{-2}\logtol2$}\\
};

\end{tikzpicture}


==> imgs/root-finding/total-work.tex <==
% This file was created by matplotlib2tikz v0.6.10.
\begin{tikzpicture}

\begin{axis}[
xlabel={Normalised $\tol$},
ylabel={Total work $\times \tol^{2}$},
xmin=1e-05, xmax=0.1,
%ymin=10000, ymax=1000000,
xmode=log,
ymode=log,
grid=both,
width=\figurewidth,
height=\figureheight,
xtick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10},
xticklabels={,$10^{-5}$,$10^{-4}$,$10^{-3}$,$10^{-2}$,$10^{-1}$,,},
ytick={1000,10000,100000,1000000,10000000},
yticklabels={,$10^{4}$,$10^{5}$,$10^{6}$,},
tick pos=both
]
\addplot [mark=*]
table {%
0.0970765528188712 406450.6484375
0.0485382764094356 130188.908203125
0.0242691382047178 75556.15625
0.0121345691023589 59540.7414550781
0.0121345691023589 118557.067626953
0.00606728455117945 71573.1125488281
0.00606728455117945 129764.010864258
0.00303364227558973 89675.6986618042
0.00151682113779486 102484.799846709
0.000758410568897431 103695.262930095
0.000379205284448716 126036.714774258
0.000189602642224358 131756.223347662
0.000189602642224358 232224.030880416
9.48013211120547e-05 172418.066484325
};
\label{root-finding/complexity-line0}
\addplot [dashed, domain=1e-6:1]
{%
%1e-05 291722.073796452
2200.8878157798435*(ln(x))^2
};
\label{root-finding/complexity-line1}
\coordinate (legend) at (axis description cs:0.97,0.97);
\end{axis}

\matrix [matrix of nodes, /pgfplots/every axis legend, inner sep=1pt,
row sep=1pt,cells={anchor=west}, text depth=0.5ex, text height=2ex,
anchor={north east}] at (legend) {
\ref{root-finding/complexity-line1}& {$\varepsilon^{-2} \logtol2$}\\
};
\end{tikzpicture}

